AutoPoly: Predicting a Polygonal Mesh Construction Sequence from a Silhouette Image

Polygonal modeling is a core task of content creation in Computer Graphics. The complexity of modeling, in terms of the number and the order of operations and time required to execute them makes it challenging to learn and execute. Our goal is to automatically derive a polygonal modeling sequence for a given target. Then, one can learn polygonal modeling by observing the resulting sequence and also expedite the modeling process by starting from the auto-generated result. As a starting point for building a system for 3D modeling in the future, we tackle the 2D shape modeling problem and present AutoPoly, a hybrid method that generates a polygonal mesh construction sequence from a silhouette image. The key idea of our method is the use of the Monte Carlo tree search (MCTS) algorithm and differentiable rendering to separately predict sequential topological actions and geometric actions. Our hybrid method can alter topology, whereas the recently proposed inverse shape estimation methods using differentiable rendering can only handle a fixed topology. Our novel reward function encourages MCTS to select topological actions that lead to a simpler shape without self-intersection. We further designed two deep learning-based methods to improve the expansion and simulation steps in the MCTS search process: an $n$-step "future action prediction" network (nFAP-Net) to generate candidates for potential topological actions, and a shape warping network (WarpNet) to predict polygonal shapes given the predicted rendered images and topological actions. We demonstrate the efficiency of our method on 2D polygonal shapes of multiple man-made object categories.

==> algos/simulation_algo.tex <==
\begin{algorithm}
\caption{An algorithm with caption}\label{alg:simulation}
\begin{algorithmic}
\Require $n \geq 0$
\Ensure $y = x^n$
\State $y \gets 1$
\State $X \gets x$
\State $N \gets n$
\While{$N \neq 0$}
\If{$N$ is even}
    \State $X \gets X \times X$
    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$
    \State $N \gets N - 1$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

==> chi/cgf/cgf_metadata.tex <==
\title[This is title...]%
      {This is title...}

\author[paperxxxx]{paperxxxx}

% \author[I-Chao Shen et al.]
% {\parbox{\textwidth}{\centering I-Chao Shen$^{1}$ ~ Kuan-Hung Liu$^{1}$ ~ Li-Wen Su$^{1}$ ~ Yu-Ting Wu$^{1}$ ~ Bing-Yu Chen$^{2}$
% %        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
%         }
%         \\
% % For Computer Graphics Forum: Please use the abbreviation of your first name.
% {\parbox{\textwidth}{\centering $^1$ \{jdily, lkh94, susan31213, kevincosner\}@cmlab.csie.ntu.edu.tw, National Taiwan University, Taiwan \\
% $^2$ robin@ntu.edu.tw, National Taiwan University, Taiwan
% %        $^2$ Another Department to illustrate the use in papers from authors
% %             with different affiliations
%       }
% }
% }

==> chi/chi_ccs_keyword.tex <==
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121.10003129</concept_id>
<concept_desc>Human-centered computing~Interactive systems and tools</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Interactive systems and tools}

==> chi/chi_metadata.tex <==
\newcommand{\name}{EvIcon}
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{This is title...}
%\title{Perception-based Design Tool for Interface Icon Set Using Data-driven Methods}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{ANONYMOUS AUTHOR(S)}
% \authornote{}
% \email{}
% \orcid{}
% \author{}
% \authornotemark[1]
% \email{}
% \affiliation{%
%   \institution{}
%   \streetaddress{}
%   \city{}
%   \state{}
%   \postcode{}
% }

==> conf_preamble.tex <==
\RequirePackage{ifthen}
\newcommand{\conf}{siggraph}
% submit, camera, final....
\newcommand{\stage}{final}
% \def\conf{cvpr}
% \input{siggraph_preamble}
\newcommand{\isequal}[3]{
    \ifthenelse{\equal{#1}{#2}}{
        #3
    }{}    
}

\isequal{\conf}{siggraph}{\input{siggraph/siggraph_preamble}}
\isequal{\conf}{cvpr}{\input{cvpr/cvpr_preamble}}
\isequal{\conf}{eccv}{\input{eccv/eccv_preamble}}
\isequal{\conf}{uist}{\input{uist/uist_preamble}}
\isequal{\conf}{chi}{\input{chi/chi_preamble}}
\isequal{\conf}{pg}{\input{cgf/cgf_preamble}}
\isequal{\conf}{tvcg}{\input{ieeetrans/ieeetrans_preamble}}

% \ifthenelse{\equal{\conf}{siggraph}}{
%     \input{siggraph/siggraph_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{cvpr}}{
%     \input{cvpr/cvpr_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{eccv}}{
%     \input{eccv/eccv_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{uist}}{
%     \input{uist/uist_preamble}
% }
% {
% }

==> cvpr/cvpr_metadata.tex <==
\title{This is title.}

\author{First author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

==> eccv/eccv_metadata.tex <==
\pagestyle{headings}
\mainmatter
\def\ECCVSubNumber{666}  % Insert your submission number here

\title{This is paper title} % Replace with your title

% INITIAL SUBMISSION 
%\begin{comment}
\titlerunning{ECCV-20 submission ID \ECCVSubNumber} 
\authorrunning{ECCV-20 submission ID \ECCVSubNumber} 
\author{Anonymous ECCV submission}
\institute{Paper ID \ECCVSubNumber}



\begin{comment}
\titlerunning{Abbreviated paper title}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
\author{First Author\inst{1}\orcidID{0000-1111-2222-3333} \and
Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
%
\authorrunning{F. Author et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{Princeton University, Princeton NJ 08544, USA \and
Springer Heidelberg, Tiergartenstr. 17, 69121 Heidelberg, Germany
\email{lncs@springer.com}\\
\url{http://www.springer.com/gp/computer-science/lncs} \and
ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
\email{\{abc,lncs\}@uni-heidelberg.de}}
\end{comment}

==> figures/blueprint_fig.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{figs/3view_0.png}
\caption{
\todo{Maybe remove.}
3D model artists often use image blueprints from different viewing directions to assist the modeling process.
The most common viewing directions used in blueprint modeling is ``top'', ``front'', and ``side''.
% The blueprint is beneficial for gaining sense of spatial awareness. 
}
\label{fig:blueprint_modeling}
\end{figure}

==> figures/qual_result.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.95\linewidth]{figs/results_shrink.pdf}
\caption{
\textbf{Qualitative evaluation after reconstructing ShapeNet shapes.}
Compared to the pure differentiable rendering method using \textit{simple} or \textit{complex} shapes, \textit{AutoPoly} generates final shapes that better match the target shape (sm), with a less complex shape (sc) and fewer self-intersections (si).
% better while keep lower shape complexity and number of self-intersection.
% In the table, ``si'' denotes the number of self-intersection, ``sm'' denotes the shape matching score, and ``sc'' denotes the shape complexity which shows (|V|, |E|, |F|).
}
\label{fig:results}
\end{figure*}

==> figures/syn_data_set.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figs/syn_img_grid.png}
\caption{
% \todo{maybe move this one to supplemental material if the page count is more than 7.}
The random generation process of synthetic shape.
At each step, we randomly choose a shape element and apply a random topological action.
Finally, we randomly deform all vertices as the random shape.
}
\label{fig:training_data}
\end{figure}

==> figures/train_data_gen.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figs/train_data_gen.pdf}
\caption{
% \todo{maybe move this one to supplemental material if the page count is more than 7.}
The random generation process of synthetic shape.
At each step, we randomly choose a shape element and apply a random topological action.
Finally, we randomly deform all vertices as the random shape.
}
\label{fig:training_data}
\end{figure}

==> old_doc/overview.tex <==
\section{Overview}
Our goal is to recover a feasible polygonal mesh construction sequence such that the final shape matches the target shape in the input images.
The construction sequence we recovered consists of both topological and geometrical actions.
Topological action represents modeling action that increases or decreases the shape elements, such as vertex, edge, and face.
In this paper, we support four different kinds of topological actions as illustrated in \Cref{fig:topo_acts}.
Conversely, geometric action only transforms the existing shape elements, such as translation, scaling, and rotation.
The problem of recovering such a construction sequence can be seen as a long-term planning problem because selecting each topological and geometric action will affect other subsequent actions.
In this work, we propose a hybrid method that recovers sequential topological and geometric actions using Monte Carlo tree search and inverse shape estimation using differentiable rendering.
\input{figures/topo_act_fig}
\input{mcts}
\input{diff_render}

==> tables/shape_quan_table.tex <==
\begin{table}[ht!]
\centering
\caption{
Quantitative evaluation on synthetic shape reconstruction.
}
\begin{tabular}[t]{lcccc}
\toprule
Method & $r_{sm}$ & $r_{sc}$ & $r_{si}$ & $r_{\text{all}}$\\
\midrule
inv shape estimate (simple)&1&2&3&\\
inv shape estimate (complex)&&&&\\
Our method &&&& \\
Our learning-based method &&&&\\
\bottomrule
\end{tabular}
\label{tab:shape_quan}
\end{table}%

==> uist/uist_ccs_keyword.tex <==
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121.10003129</concept_id>
<concept_desc>Human-centered computing~Interactive systems and tools</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Interactive systems and tools}

==> uist/uist_metadata.tex <==
\newcommand{\name}{EvIcon}
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{This is title...}
%\title{Perception-based Design Tool for Interface Icon Set Using Data-driven Methods}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{ANONYMOUS AUTHOR(S)}
% \authornote{}
% \email{}
% \orcid{}
% \author{}
% \authornotemark[1]
% \email{}
% \affiliation{%
%   \institution{}
%   \streetaddress{}
%   \city{}
%   \state{}
%   \postcode{}
% }
